ListT5: Listwise Reranking with Fusion-in-Decoder Improves Zero-shot Retrieval

We propose ListT5, a novel reranking approach based on Fusion-in-Decoder (FiD) that handles multiple candidate passages at both train and inference time. We also introduce an efficient inference framework for listwise ranking based on m-ary tournament sort with output caching. We evaluate and compare our model on the BEIR benchmark for zero-shot retrieval task, demonstrating that ListT5 (1) outperforms the state-of-the-art RankT5 baseline with a notable +1.3 gain in the average NDCG@10 score, (2) has an efficiency comparable to pointwise ranking models and surpasses the efficiency of previous listwise ranking models, and (3) overcomes the lost-in-the-middle problem of previous listwise rerankers. Our code, model checkpoints, and the evaluation framework are fully open-sourced at \url{https://github.com/soyoung97/ListT5}.

==> figure/fig_inference_main.tex <==
\begin{figure}[!t]
{
\centering
    \includegraphics[width=\columnwidth]{imgs/inference_illustration_higher.png}
    \caption{Illustration of our inference scenario. Our method works as a local aggregator which aggreates to 1(Top1) or 2(Top2) passages, and it iterates through multiple inference to rerank top 10 results from first-stage retrieval results. Output caching effectively reduces the number of total forwards. \red{conerns: (1) Does this figure overall understands well?}
    \red{include output sequence 5}
    }
    \label{fig:inference_main}
}
\end{figure}


==> figure/fig_pareto.tex <==
\begin{figure}[!]
{
\centering
    \includegraphics[width=\columnwidth]{imgs/first_inference_with_pareto.png }
    \caption{We aim to improve the Pareto front of the performance (avg. in BeIR) and efficiency (FLOPs) in zero-shot retrieval.}
    \label{fig:fig_pareto}
}
\end{figure}


==> figure/fig_placeholder_ablation.tex <==
\begin{figure}[!t]
{
\centering
    \includegraphics[width=\columnwidth]{imgs/fig_placeholder_ablation.png}
    \caption{Ablation results on varying the generation order of passages. We can see that generating from the least relevant passages shows better average performance on beir.}
    \label{fig:fig_ablation}
}
\end{figure}


==> figure/fig_placeholder_main.tex <==
\begin{figure*}[t]
{
\centering
    \includegraphics[width=\textwidth]{imgs/placeholder_table.png}
    \caption{Main results. \red{Concerns: 1. add/remove gpt3.5 results? 2. In-domain results are not better than baseline, but they still give insights, but it's not our focus(our focus is out-domain) remove in-domain results? 3. display only ours best (get top2), or display both?
}}
    \label{fig:fig_placeholder_main}
}
\end{figure*}


==> table/beir_table.tex <==
\begin{table*}[t!]
    \small
    \resizebox{\textwidth}{!}{\begin{tabular}{l | c | c c c | c c c c | c | c}
        \toprule
        \multicolumn{1}{l}{\textbf{Model ($\rightarrow$)}} &
        \multicolumn{1}{c}{Lexical}   &
        \multicolumn{3}{c}{Sparse}   &
        \multicolumn{4}{c}{Dense} &
        \multicolumn{1}{c}{Late-Interaction} &
        \multicolumn{1}{c}{Re-ranking} \\ 
        \cmidrule(lr){1-1}
        \cmidrule(lr){2-2}
        \cmidrule(lr){3-5}
        \cmidrule(lr){6-9}
        \cmidrule(lr){10-10}
        \cmidrule(lr){11-11}
        \multicolumn{1}{l}{\textbf{Dataset ($\downarrow$)}} &
        \multicolumn{1}{c}{\textbf{BM25}} &
        \multicolumn{1}{c}{\textbf{DeepCT}} &
        \multicolumn{1}{c}{\textbf{SPARTA}} &
        \multicolumn{1}{c}{\textbf{docT5query}} &
        \multicolumn{1}{c}{\textbf{DPR}} &
        \multicolumn{1}{c}{\textbf{ANCE}} &
        \multicolumn{1}{c}{\textbf{TAS-B}} &
        \multicolumn{1}{c}{\textbf{GenQ}} &
        \multicolumn{1}{c}{\textbf{ColBERT}} &
        \multicolumn{1}{c}{\textbf{BM25+CE}} \\
        \midrule

   MS MARCO & 0.228 & 0.296$^\ddagger$ & 0.351$^\ddagger$ & 0.338$^\ddagger$ & 0.177 & 0.388$^\ddagger$ & 0.408$^\ddagger$ & 0.408$^\ddagger$ & \underline{0.401}$^\ddagger$ & \textbf{0.413}$^\ddagger$ \\  \midrule \midrule
   
   TREC-COVID    & 0.656 & 0.406 & 0.538 & \underline{0.713} & 0.332& 0.654 & 0.481 & 0.619 & 0.677 & \textbf{0.757}\\
   BioASQ        & 0.465 & 0.407 & 0.351 & \textcolor{black}{0.431} & 0.127 & 0.306 & 0.383 & 0.398 & \underline{0.474} & \textbf{0.523} \\
   NFCorpus      & 0.325 & 0.283 & 0.301 & \underline{0.328} & 0.189 & 0.237 & 0.319 & 0.319 & 0.305 & \textbf{0.350} \\ \midrule
   NQ            & 0.329 & 0.188 & 0.398 & 0.399 & 0.474$^\ddagger$ & 0.446 & 0.463 & 0.358 & \underline{0.524} & \textbf{0.533} \\ 
   HotpotQA      & \underline{0.603} & 0.503 & 0.492 & 0.580 & 0.391 & 0.456 & 0.584 & 0.534 & 0.593 & \textbf{0.707} \\ 
   FiQA-2018     & 0.236 & 0.191 & 0.198 & 0.291 & 0.112 & 0.295 & 0.300 & 0.308 & \underline{0.317} & \textbf{0.347} \\ \midrule
   Signal-1M (RT)& \underline{0.330} & 0.269 & 0.252 & 0.307 & 0.155 & 0.249 & 0.289 & 0.281 & 0.274 & \textbf{0.338} \\ \midrule
   TREC-NEWS     & 0.398 & 0.220 & 0.258 & \underline{0.420} & 0.161 & 0.382 & 0.377 & 0.396 & 0.393 & \textbf{0.431} \\
   Robust04     & 0.408 & 0.287 & 0.276 & \underline{0.437} & 0.252 & 0.392 & 0.427 & 0.362 & 0.391 & \textbf{0.475} \\ \midrule
   ArguAna       & 0.315 & 0.309 & 0.279 & 0.349 & 0.175& 0.415 & \underline{0.429} & \textbf{0.493} & 0.233 & 0.311 \\  
   Touch\'e-2020 & \textbf{0.367} & 0.156 & 0.175 & \underline{0.347} & 0.131 & 0.240 & 0.162 & 0.182 & 0.202 & 0.271 \\ \midrule 
   CQADupStack   & 0.299 & 0.268 & 0.257 & 0.325 & 0.153 & 0.296 & 0.314 & 0.347 & \underline{0.350} & \textbf{0.370} \\
   Quora         & 0.789 & 0.691 & 0.630 & 0.802 & 0.248 & \underline{0.852} & 0.835 & 0.830 & \textbf{0.854} & 0.825 \\ \midrule
   DBPedia       & 0.313  & 0.177 & 0.314 & 0.331 & 0.263 & 0.281 & 0.384 & 0.328 & \underline{0.392} & \textbf{0.409} \\ \midrule
   SCIDOCS       & 0.158 & 0.124 & 0.126 & \underline{0.162} & 0.077 & 0.122 & 0.149 & 0.143 & 0.145 & \textbf{0.166} \\ \midrule
   FEVER         & 0.753 & 0.353 & 0.596 & \textcolor{black}{0.714} & 0.562& 0.669 & 0.700 & 0.669 & \underline{0.771} & \textbf{0.819} \\ 
   Climate-FEVER & 0.213 & 0.066 & 0.082 & 0.201 & 0.148 & 0.198 & \underline{0.228} & 0.175 & 0.184 & \textbf{0.253}\\ 
   SciFact       & 0.665 & 0.630 & 0.582 & \underline{0.675} & 0.318 & 0.507 & 0.643 & 0.644 & 0.671 & \textbf{0.688} \\ \midrule
   \multicolumn{2}{c|}{Avg. Performance vs. BM25} & \textbf{- 27.9\%} & \textbf{- 20.3\%} & \textbf{+ 1.6\%} & \textbf{- 47.7\%} & \textbf{- 7.4\%} & \textbf{ - 2.8\%} & \textbf{ - 3.6\%} & \textbf{+ 2.5\%} & \textbf{+ 11\%} \\ 
        \bottomrule
    \end{tabular}}
    \caption{In-domain and zero-shot performances on \beir benchmark. All scores denote \textbf{nDCG@10}. The best score on a given dataset is marked in \textbf{bold}, and the second best is \underline{underlined}. Corresponding Recall@100 performances can be found in Table \ref{tab:results-recall}. $\ddagger$ indicates the in-domain performances. \vspace{-5mm}}
    \label{tab:results}
\end{table*}

==> table/draft1_table.tex <==
\begin{table*}[t!]
\small
\resizebox{\textwidth}{!}{
%\renewcommand{\arraystretch}{1.15}


\begin{tabular}{@{}ll|ccccc|ccccc@{}}
\toprule
\multicolumn{2}{r|}{First-stage retrieval by:} &
  \multicolumn{5}{c|}{BM25 Top100} &
  \multicolumn{5}{c}{COCO-DR Large Top100} \\ \midrule
 &
   &
  \multicolumn{3}{c}{Baselines} &
  \multicolumn{2}{c|}{Ours} &
  \multicolumn{3}{c}{Baselines} &
  \multicolumn{2}{c}{Ours} \\ \cmidrule(lr){3-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(l){11-12} 
\multicolumn{1}{c}{Task (Domain)} &
  \multicolumn{1}{c|}{Dataset} &
  \begin{tabular}[c]{@{}c@{}}BM25\\ (Initial)\end{tabular} &
  MonoT5 &
  RankT5 &
  ListT5 &
  ListT5-2 &
  \begin{tabular}[c]{@{}c@{}}COCO-DR\\ (Initial)\end{tabular} &
  MonoT5 &
  RankT5 &
  ListT5 &
  ListT5-2 \\ \midrule
\multicolumn{1}{l|}{\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Passage\\ Retrieval\end{tabular}}} &
  MS MARCO &
  22.8 &
  40.0 &
  \textbf{40.8} &
  40.7 &
  40.7 &
  41.9 &
  44.2 &
  \textbf{46.4} &
  \textbf{46.4} &
  46.3 \\
\multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{+ top1000} &
  22.8 &
  43.6 &
  44.7 &
  44.7 &
  \textbf{44.9} &
  41.9 &
  43.1 &
  43.1 &
  46.1 &
  \textbf{46.2} \\
\multicolumn{1}{l|}{} &
  TREC-DL19 &
  50.6 &
  71.5 &
  \textbf{72.4} &
  71.2 &
  71.8 &
   &
   &
   &
   &
   \\
\multicolumn{1}{l|}{} &
  TREC-DL20 &
  48.0 &
  67.0 &
  \textbf{68.3} &
  67.3 &
  68.1 &
   &
   &
   &
   &
   \\ \midrule
\multicolumn{2}{c|}{\textbf{In-domain average}} &
  36.1 &
  55.5 &
  \textbf{56.6} &
  56.0 &
  56.4 &
  41.9 &
  43.7 &
  44.8 &
  \textbf{46.3} &
  \textbf{46.3} \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Bio-Medical\\ Information\\ Retrieval\end{tabular}}} &
  TREC-COVID &
  59.5 &
  \textbf{78.3} &
  77.7 &
  76.7 &
  \textbf{78.3} &
  80.8 &
  \textbf{83.5} &
  \textbf{83.5} &
  83.2 &
  \textbf{83.5} \\
\multicolumn{1}{l|}{} &
  NFCorpus &
  32.2 &
  \textbf{35.7} &
  35.1 &
  35.5 &
  35.6 &
  35.5 &
  35.6 &
  35.5 &
  \textbf{36.2} &
  \textbf{36.2} \\
\multicolumn{1}{l|}{} &
  BioASQ &
  52.2 &
  55.3 &
  \textbf{58.2} &
  57.2 &
  56.4 &
   &
   &
   &
   &
   \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Question\\ Answering\\ (QA)\end{tabular}}} &
  NQ &
  30.5 &
  52.1 &
  \textbf{53.2} &
  52.0 &
  53.1 &
  54.3 &
  57.9 &
  59.6 &
  59.7 &
  60.0 \\
\multicolumn{1}{l|}{} &
  HotpotQA &
  63.3 &
  71.2 &
  \textbf{72.8} &
  72.1 &
  72.6 &
  63.3 &
  68.7 &
  \textbf{71.1} &
  70.3 &
  70.9 \\
\multicolumn{1}{l|}{} &
  FiQA-2018 &
  23.6 &
  39.2 &
  39.2 &
  39.5 &
  \textbf{39.6} &
  32.3 &
  41.2 &
  41.3 &
  \textbf{41.7} &
  \textbf{41.7} \\ \midrule
\multicolumn{1}{l|}{Tweet Retrieval} &
  Signal-1M (RT) &
  33.0 &
  32.0 &
  30.8 &
  33.3 &
  \textbf{33.5} &
   &
   &
   &
   &
   \\ \midrule
\multicolumn{1}{l|}{\multirow{2}{*}{News Retrieval}} &
  TREC-NEWS &
  39.5 &
  48.0 &
  45.4 &
  47.9 &
  \textbf{48.5} &
   &
   &
   &
   &
   \\
\multicolumn{1}{l|}{} &
  Robust04 &
  40.7 &
  53.4 &
  \textbf{54.3} &
  52.0 &
  52.1 &
   &
   &
   &
   &
   \\ \midrule
\multicolumn{1}{l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Argument\\ Retrieval\end{tabular}}} &
  Arguana &
  40.8 &
  34.4 &
  35.5 &
  \textbf{49.7} &
  48.9 &
  46.9 &
  33.0 &
  34.8 &
  49.0 &
  \textbf{49.3} \\
\multicolumn{1}{l|}{} &
  Touche-2020 &
  44.2 &
  29.6 &
  \textbf{37.1} &
  34.2 &
  33.4 &
  21.6 &
  25.7 &
  \textbf{35.7} &
  29.1 &
  29.6 \\ \midrule
\multicolumn{1}{l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Duplicate Q.\\ Retrieval\end{tabular}}} &
  CQADupStack &
  30.0 &
  38.6 &
  37.0 &
  38.4 &
  \textbf{38.8} &
  37.3 &
  40.5 &
  38.7 &
  40.7 &
  \textbf{40.9} \\
\multicolumn{1}{l|}{} &
  Quora &
  78.9 &
  84.6 &
  83.3 &
  86.1 &
  \textbf{86.4} &
  \textbf{87.3} &
  84.0 &
  83.0 &
  86.2 &
  86.3 \\ \midrule
\multicolumn{1}{l|}{Entity Retrieval} &
  DBPedia &
  31.8 &
  42.8 &
  43.7 &
  \textbf{43.9} &
  43.7 &
  40.7 &
  44.4 &
  \textbf{46.1} &
  45.6 &
  45.4 \\ \midrule
\multicolumn{1}{l|}{Citation Pred.} &
  SCIDOCS &
  14.9 &
  16.7 &
  16.8 &
  17.2 &
  \textbf{17.6} &
  17.3 &
  17.5 &
  17.5 &
  17.7 &
  \textbf{18.3} \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{Fact Checking}} &
  FEVER &
  65.2 &
  78.4 &
  77.6 &
  77.8 &
  \textbf{79.8} &
  74.9 &
  78.9 &
  79.7 &
  79.8 &
  \textbf{81.4} \\
\multicolumn{1}{l|}{} &
  Climate-FEVER &
  16.5 &
  23.1 &
  21.2 &
  22.8 &
  \textbf{24.0} &
  23.1 &
  24.2 &
  22.9 &
  23.9 &
  \textbf{24.9} \\
\multicolumn{1}{l|}{} &
  SciFact &
  67.9 &
  73.1 &
  73.5 &
  \textbf{74.1} &
  \textbf{74.1} &
  71.9 &
  73.5 &
  73.6 &
  \textbf{74.4} &
  74.3 \\ \midrule
\multicolumn{2}{c|}{\textbf{BeIR average}} &
  42.5 &
  49.3 &
  49.6 &
  50.6 &
  \textbf{50.9} &
  47.1 &
  48.4 &
  49.5 &
  50.6 &
  \textbf{50.9} \\ \bottomrule
\end{tabular}




}
\caption{main result. All results are run in our same setup using the released checkpoint. \red{Concerns: 2. In-domain results are not better than baseline, but they still give insights, but it's not our focus(our focus is out-domain) remove in-domain results? 3. display only ours best (get top2), or display both?} S.C means the second chance variant of \textsc{ListT5}.}
\label{table/draft1_table}
\end{table*}

==> table/draft_table.tex <==
\begin{table*}[t!]
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|l|ccc|ccr@{}}
\toprule
\multirow{2}{*}{Task} & \multirow{2}{*}{Dataset} & \multicolumn{3}{c|}{Baselines} & \multicolumn{3}{c}{Ours (Sort 5)} \\ \cmidrule(l){3-8} 
                      &                          & BM25 & MonoT5 & RankT5 & Top1 & Top2 & + \\ \midrule
\multirow{4}{*}{Passage R.}     & MS MARCO       & 22.8 & 40.0   & \textbf{40.8}   & 40.7     & 40.7     & 0.0  \\
                                & + top1000     & 22.8 & 43.6   & \textbf{44.7}   & 44.7     & -        & -    \\
                                & TREC-DL19      & 50.6 & 71.5   & \textbf{72.4}   & 71.2     & 71.8     & 0.6  \\
                                & TREC-DL20      & 48.0 & 67.0   & \textbf{68.3}   & 67.3     & 68.1     & 0.8  \\ \midrule
\multicolumn{2}{c|}{In-domain avg.}              & 36.1 & 55.5   & \textbf{56.6}   & 56.0     & -        & -    \\ \midrule[1.5pt]
\multirow{3}{*}{Bio-Medical IR} & TREC-COVID     & 59.5 & \textbf{78.3}   & 77.7   & 76.7     & 78.3     & 1.6  \\
                                & NFCorpus       & 32.2 & 35.7   & 35.1   & 35.5     & \textbf{35.6}     & 0.1  \\
                                & BioASQ         & 52.2 & 55.3   & \textbf{58.2}   & 57.2     & 56.4     & -0.8 \\
\midrule
\multirow{3}{*}{QA}             & NQ             & 30.5 & 52.1   & \textbf{53.2}   & 52.0     & 53.1     & 1.1  \\
                                & HotpotQA       & 63.3 & 71.2   & \textbf{72.8}   & 72.1     & 72.6     & 0.5  \\
                                & FiQA-2018      & 23.6 & 39.2   & 39.2   & 39.5     & \textbf{39.6}     & 0.1  \\
\midrule
Tweet R.                        & Signal-1M (RT) & 33.0 & 32.0   & 30.8   & 33.3     & \textbf{33.5}     & 0.2  \\
\midrule
\multirow{2}{*}{News R.}        & TREC-NEWS      & 39.5 & 48.0   & 45.4   & 47.9     & \textbf{48.5}     & 0.6  \\
                                & Robust04       & 40.7 & 53.4   & \textbf{54.3}   & 52.0     & 52.1     & 0.1  \\
\midrule
\multirow{2}{*}{Argument R.}    & Arguana        & 40.8 & 34.4   & 35.5   & \textbf{49.7}     & 48.9     & -0.8 \\
                                & Touche-2020    & 44.2 & 29.6   & 37.1   & 34.2     & 33.4     & -0.8 \\
\midrule
\multirow{2}{*}{Duplicate Q R.} & CQADupStack    & 30.0 & 38.6   & 37.0   & 38.4     & \textbf{38.8}     & 0.4  \\
                                & Quora          & 78.9 & 84.6   & 83.3   & \textbf{86.1}     & 86.4     & 0.3  \\
\midrule
Entity R.                       & DBPedia        & 31.8 & 42.8   & \textbf{43.7}   & 43.9     & 43.7     & -0.2 \\
\midrule
Citation Pred.                  & SCIDOCS        & 14.9 & 16.7   & 16.8   & \textbf{17.2}     & 17.6     & 0.4  \\
\midrule
\multirow{3}{*}{Fact Checking}  & FEVER          & 65.2 & 78.4   & 77.6   & 77.8     & \textbf{79.8}     & 2.0  \\
                                & Climate-FEVER  & 16.5 & 23.1   & 21.2   & 22.8     & \textbf{24.0}     & 1.2  \\
                                & SciFact        & 67.9 & 73.1   & \textbf{73.5}   & 74.1     & 74.1     & 0.0  \\ \midrule[\heavyrulewidth]
\multicolumn{2}{c|}{BeIR avg.}                   & 42.5 & 49.3   & 49.6   & 50.6     & \textbf{50.9}     & 0.3  \\ \bottomrule
\end{tabular}}
\end{table*}

%\heavyrulewidth

==> table/main_table_before.tex <==
\begin{table*}[t!]

\centering
%\small\addtolength{\tabcolsep}{0pt}
%\fontsize{7}{7}\selectfont
%\renewcommand{\arraystretch}{1.05}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|cccc|ccc|cccc@{}}
\toprule
 &
  \multicolumn{4}{c|}{BM25 Top100} &
  \multicolumn{3}{c|}{BM25 Top100 + 3B models} &
  \multicolumn{4}{c}{COCO-DR (Large) Top100} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-12}
\multicolumn{1}{c|}{Dataset} &
  Initial &
  MonoT5 &
  RankT5 &
  \begin{tabular}[c]{@{}c@{}}\textbf{ListT5}\\\textbf{($\mathbf{r = 2}$})\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}MonoT5-\\ 3B\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}RankT5-\\ 3B\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{ListT5-3B}\\\textbf{($\mathbf{r = 2}$)}\end{tabular} &
  Initial &
  MonoT5 &
  RankT5 &
  \begin{tabular}[c]{@{}c@{}}\textbf{ListT5}\\ \textbf{($\mathbf{r = 2}$)}\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}l@{}}MS MARCO\\ (Top1000)\end{tabular} &
  22.8 &
  43.6 &
  44.7 &
  \textbf{44.9} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c|}{-} &
  41.9 &
  43.1 &
  46.2 &
  \textbf{46.3} \\ \midrule
TREC-COVID &
  59.5 &
  \textbf{78.3} &
  77.7 &
  \textbf{78.3} &
  79.8 &
  81.7 &
  \textbf{\textbf{84.7}} &
  80.8 &
  \textbf{83.5} &
  \textbf{83.5} &
  \textbf{83.5} \\
NFCorpus &
  32.2 &
  \textbf{35.7} &
  35.1 &
  35.6 &
  37.3 &
  \textbf{37.4} &
  37.7 &
  35.5 &
  35.6 &
  35.5 &
  \textbf{36.2} \\
BioASQ &
  52.2 &
  55.3 &
  \textbf{58.2} &
  56.4 &
  57.5 &
  \textbf{58.3} &
  \textbf{58.3} &
  - &
  - &
  - &
  - \\
NQ &
  30.5 &
  52.1 &
  \textbf{53.2} &
  53.1 &
  56.4 &
  \textbf{57.8} &
  56.2 &
  54.3 &
  57.9 &
  59.6 &
  \textbf{60.0} \\
HotpotQA &
  63.3 &
  71.2 &
  \textbf{72.8} &
  72.6 &
  74.3 &
  74.8 &
  \textbf{75.6} &
  63.3 &
  68.7 &
  \textbf{71.1} &
  70.9 \\
FiQA-2018 &
  23.6 &
  39.2 &
  39.2 &
  \textbf{39.6} &
  \textbf{46.0} &
  45.2 &
  45.1 &
  32.3 &
  41.2 &
  41.3 &
  \textbf{41.7} \\
Signal-1M (RT) &
  33.0 &
  32.0 &
  30.8 &
  \textbf{\red{33.5}} &
  32.2 &
  31.9 &
  \textbf{33.8} &
  - &
  - &
  - &
  - \\
TREC-NEWS &
  39.5 &
  48.0 &
  45.4 &
  \textbf{48.5} &
  48.3 &
  49.5 &
  \textbf{53.2} &
  - &
  - &
  - &
  - \\
Robust04 &
  40.7 &
  53.4 &
  \textbf{54.3} &
  52.1 &
  \textbf{58.5} &
  58.3 &
  57.8 &
  - &
  - &
  - &
  - \\
Arguana &
  40.8 &
  34.4 &
  35.5 &
  \textbf{\red{48.9}} &
  46.8 &
  37.4 &
  \textbf{50.6} &
  46.9 &
  33.0 &
  34.8 &
  \textbf{49.3} \\
Touche-2020 &
  \textbf{44.2} &
  29.6 &
  37.1 &
  33.4 &
  32.5 &
  \textbf{38.8} &
  33.6 &
  21.6 &
  25.7 &
  \textbf{35.7} &
  29.6 \\
CQADupStack &
  30.0 &
  38.6 &
  37.0 &
  \textbf{38.8} &
  41.3 &
  40.3 &
  \textbf{42.1} &
  37.3 &
  40.5 &
  38.7 &
  \textbf{40.9} \\
Quora &
  78.9 &
  84.6 &
  83.3 &
  \textbf{\red{86.4}} &
  84.0 &
  83.6 &
  \textbf{86.9} &
  \textbf{87.3} &
  84.0 &
  83.0 &
  86.3 \\
DBPedia &
  31.8 &
  42.8 &
  \textbf{43.7} &
  \textbf{43.7} &
  44.8 &
  45.0 &
  \textbf{46.2} &
  40.7 &
  44.4 &
  \textbf{46.1} &
  45.4 \\
SCIDOCS &
  14.9 &
  16.7 &
  16.8 &
  \textbf{17.6} &
  19.0 &
  18.9 &
  \textbf{19.5} &
  17.3 &
  17.5 &
  17.5 &
  \textbf{18.3} \\
FEVER &
  65.2 &
  78.4 &
  77.6 &
  \textbf{79.8} &
  80.0 &
  79.8 &
  \textbf{82.0} &
  74.9 &
  78.9 &
  79.7 &
  \textbf{81.4} \\
Climate-FEVER &
  16.5 &
  23.1 &
  21.2 &
  \textbf{24.0} &
  \textbf{26.2} &
  24.5 &
  24.8 &
  23.1 &
  24.2 &
  22.9 &
  \textbf{24.9} \\
SciFact &
  67.9 &
  73.1 &
  73.5 &
  \textbf{74.1} &
  76.3 &
  \textbf{77.1} &
  77.0 &
  71.9 &
  73.5 &
  73.6 &
  \textbf{74.3} \\ \midrule
\textbf{Avg (BEIR)} &
  42.5 &
  49.3 &
  49.6 &
  \textbf{50.9} &
  52.3 &
  52.2 &
  \textbf{53.6} &
  49.1 &
  50.6 &
  51.6 &
  \textbf{53.1} \\ \bottomrule
\end{tabular}
}
\caption{Comparison of \textsc{ListT5} against \textbf{pointwise} ranking models, on MS MARCO dev set and BEIR, in NDCG@10.
MS MARCO-Top1000 results for 3B models are omitted due to their long inference time. \textsc{ListT5}-base excels in both performance and model size (than MonoT5-3B or RankT5-3B) for datasets in \red{red}.}
\label{table/main_table_before}

\end{table*}



==> table/main_table_deprecated.tex <==
\begin{table*}[t!]

\centering
\small\addtolength{\tabcolsep}{0pt}
\fontsize{6}{6}\selectfont
\renewcommand{\arraystretch}{1.05}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multicolumn{1}{l|}{}               & \multicolumn{4}{c|}{BM25 Top100}                                          & \multicolumn{4}{c}{COCO-DR Top100}                   \\ \cmidrule(lr){2-5} \cmidrule(l){6-9} 
\multicolumn{1}{c|}{Dataset} &
  \begin{tabular}[c]{@{}c@{}}Initial\\ (BM25)\end{tabular} &
  MonoT5 &
  RankT5 &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{ListT5}\\ \textbf{(r = 2)}\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}Initial\\ (COCO-DR)\end{tabular} &
  MonoT5 &
  RankT5 &
  \begin{tabular}[c]{@{}c@{}}\textbf{ListT5}\\ \textbf{(r = 2)}\end{tabular} \\ \midrule
%\multicolumn{9}{l}{In-domain performance}                                                                                                                              \\ \midrule
%\multicolumn{1}{l|}{MS MARCO}       & 22.8 & 40.0          & 40.8          & \multicolumn{1}{c|}{40.7}          & 41.9          & 44.2 & \textbf{46.4} & 46.3          \\
\multicolumn{1}{l|}{\begin{tabular}[l]{@{}l@{}}MS MARCO\\ (Top1000)\end{tabular}}    & 22.8 & 43.6          & 44.7          & \multicolumn{1}{c|}{\textbf{44.9}} & 41.9          & 43.1 & 46.2          & \textbf{46.3} \\ \midrule

%\multicolumn{1}{l|}{TREC-DL19}      & 50.6 & 71.5          & \textbf{72.4} & \multicolumn{1}{c|}{71.8}          &               &      &               &               \\

%\multicolumn{1}{l|}{TREC-DL20}      & 48.0 & 67.0          & \textbf{68.3} & \multicolumn{1}{c|}{68.1}          &               &      &               &               \\ \midrule
%\multicolumn{1}{l|}{Avg.}           & 36.1 & 55.5          & \textbf{56.6} & \multicolumn{1}{c|}{56.4}          & 41.9          & 43.7 & 44.8          & \textbf{46.3} \\ \midrule
%\multicolumn{9}{l}{Out-domain performance (on BeIR)}                                                                                                                   \\ \midrule
\multicolumn{1}{l|}{TREC-COVID} &
  59.5 &
  \textbf{78.3} &
  77.7 &
  \multicolumn{1}{c|}{\textbf{78.3}} &
  80.8 &
  \textbf{83.5} &
  \textbf{83.5} &
  \textbf{83.5} \\
\multicolumn{1}{l|}{NFCorpus}       & 32.2 & \textbf{35.7} & 35.1          & \multicolumn{1}{c|}{35.6}          & 35.5          & 35.6 & 35.5          & \textbf{36.2} \\
\multicolumn{1}{l|}{BioASQ}         & 52.2 & 55.3          & \textbf{58.2} & \multicolumn{1}{c|}{56.4}          &        $-$      &   $-$  &     $-$       &    $-$            \\
\multicolumn{1}{l|}{NQ}             & 30.5 & 52.1          & \textbf{53.2} & \multicolumn{1}{c|}{53.1}          & 54.3          & 57.9 & 59.6          & \textbf{60.0}          \\
\multicolumn{1}{l|}{HotpotQA}       & 63.3 & 71.2          & \textbf{72.8} & \multicolumn{1}{c|}{72.6}          & 63.3          & 68.7 & \textbf{71.1} & 70.9          \\
\multicolumn{1}{l|}{FiQA-2018}      & 23.6 & 39.2          & 39.2          & \multicolumn{1}{c|}{\textbf{39.6}} & 32.3          & 41.2 & 41.3          & \textbf{41.7} \\
\multicolumn{1}{l|}{Signal-1M (RT)} & 33.0 & 32.0          & 30.8          & \multicolumn{1}{c|}{\textbf{33.5}} &      $-$       & $-$  &     $-$     &         $-$  \\
\multicolumn{1}{l|}{TREC-NEWS}      & 39.5 & 48.0          & 45.4          & \multicolumn{1}{c|}{\textbf{48.5}}      &            $-$    &  $-$     &           $-$     &      $-$          \\
\multicolumn{1}{l|}{Robust04}       & 40.7 & 53.4          & \textbf{54.3} & \multicolumn{1}{c|}{52.1}          &       $-$  &   $-$    &        $-$        &        $-$        \\
\multicolumn{1}{l|}{Arguana}        & 40.8 & 34.4          & 35.5          & \multicolumn{1}{c|}{\textbf{48.9}}          & 46.9          & 33.0 & 34.8          & \textbf{49.3} \\
\multicolumn{1}{l|}{Touche-2020}    & 44.2 & 29.6          & \textbf{37.1} & \multicolumn{1}{c|}{33.4}          & 21.6          & 25.7 & \textbf{35.7} & 29.6          \\
\multicolumn{1}{l|}{CQADupStack}    & 30.0 & 38.6          & 37.0          & \multicolumn{1}{c|}{\textbf{38.8}} & 37.3          & 40.5 & 38.7          & \textbf{40.9} \\
\multicolumn{1}{l|}{Quora}          & 78.9 & 84.6          & 83.3          & \multicolumn{1}{c|}{\textbf{86.4}} & \textbf{87.3} & 84.0 & 83.0          & 86.3          \\
\multicolumn{1}{l|}{DBPedia}        & 31.8 & 42.8          & \textbf{43.7}          & \multicolumn{1}{c|}{\textbf{43.7}}          & 40.7          & 44.4 & \textbf{46.1} & 45.4          \\
\multicolumn{1}{l|}{SCIDOCS}        & 14.9 & 16.7          & 16.8          & \multicolumn{1}{c|}{\textbf{17.6}} & 17.3          & 17.5 & 17.5          & \textbf{18.3} \\
\multicolumn{1}{l|}{FEVER}          & 65.2 & 78.4          & 77.6          & \multicolumn{1}{c|}{\textbf{79.8}} & 74.9          & 78.9 & 79.7          & \textbf{81.4} \\
\multicolumn{1}{l|}{Climate-FEVER}  & 16.5 & 23.1          & 21.2          & \multicolumn{1}{c|}{\textbf{24.0}} & 23.1          & 24.2 & 22.9          & \textbf{24.9} \\
\multicolumn{1}{l|}{SciFact}        & 67.9 & 73.1          & 73.5          & \multicolumn{1}{c|}{\textbf{74.1}} & 71.9          & 73.5 & 73.6          & \textbf{74.3}          \\ \midrule
\multicolumn{1}{l|}{\textbf{Avg (BeIR)}}           & 42.5 & 49.3          & 49.6          & \multicolumn{1}{c|}{\textbf{50.9}} & 49.1          & 50.6 & 51.6          & \textbf{53.1} \\ \bottomrule
\end{tabular}

}
\caption{NDCG@10 values for MS MARCO dev set and BeIR. All results are run in the same setup using the released checkpoint.
}
\label{table/main_table}

\end{table*}



==> table/permutation_consistency.tex <==
\begin{table}
%\small\addtolength{\tabcolsep}{-4pt}
%\fontsize{6}{6}\selectfont
    \resizebox{\columnwidth}{!}
    {
\begin{tabular}{@{}l|l|cccccc|c@{}}
\toprule
 &
   &
  \multicolumn{6}{c|}{\begin{tabular}[c]{@{}c@{}}Accuracy when positive passage\\ is at index #:\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Aggre-\\ -ment \\ ratio (\uparrow)\end{tabular}} \\ \cmidrule(r){1-8}
Dataset               & Model  & 1    & 2    & 3    & 4    & 5    & Std. (\downarrow) &               \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}TREC-\\ COVID\end{tabular}} &
  GPT3.5 &
  81.6 &
  63.3 &
  75.5 &
  67.3 &
  61.2 &
  7.7 &
  55.1 \\
                      & GPT4   & 95.9 & 83.7 & 73.5 & 77.6 & 71.4 & 8.8               & 69.4          \\
                      & DuoT5  & 91.3 & 76   & x    & x    & x    & 7.7               & 79.6          \\
                      & ListT5 & 93.9 & 87.8 & 83.7 & 85.7 & 81.6 & \textbf{4.2}      & \textbf{83.7} \\ \midrule
\multirow{4}{*}{FiQA} & GPT3.5 & 90.9 & 80.4 & 78.5 & 63.8 & 64.3 & 10.3              & 60.5          \\
                      & GPT4   & 94.6 & 90.5 & 84.4 & 86.8 & 84.8 & 3.9               & 82.8          \\
                      & DuoT5  & 89.9 & 76.9 & x    & x    & x    & 6.5               & 78.1          \\
                      & ListT5 & 85.3 & 85.6 & 82.2 & 83.3 & 82.6 & \textbf{1.4}      & \textbf{90.4} \\ \bottomrule
\end{tabular}
}
\caption{Positional robustness on varying the index of positive passages on the FiQA-2018 test set. We can see that using FiD can effectively mitigate the problem of the positional bias of positive passages (lower standard deviation) with a higher agreement ratio.}
\label{table/permutation_consistency}

\end{table}

% 이런걸 측정하기 위해서 Prompt만 바꿔서 간단하게
% Rankgpt 간단하게


==> table/rankgpt-duot5_table.tex <==
\begin{table}[t]
\small\addtolength{\tabcolsep}{-3pt}
\fontsize{6}{6}\selectfont
    \resizebox{\columnwidth}{!}
    {
\renewcommand{\arraystretch}{1.05}

\begin{tabular}{@{}l|cccc@{}}
\toprule
\textbf{} &
  %\multicolumn{1}{c}{MonoT5} &
  \multicolumn{1}{c}{DuoT5} &
  \multicolumn{1}{c}{RankGPT} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}l@{}}ListT5\\($r$=1)\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}l@{}}ListT5\\($r$=2)\end{tabular}} \\ \midrule
TREC-DL19        & 71.4 & 65.8 & 71.2 & \textbf{71.8}          \\
TREC-DL20        & 67.4 & 62.9 & 67.3 & \textbf{68.1}          \\ \midrule
TREC-COVID       & \textbf{80.1} & 76.7 & 76.7 & 78.3          \\
NFCorpus         & 35.0 & \textbf{35.6} & 35.5 & \textbf{35.6}          \\
Signal-1M (RT)  & 31.4 & 32.1 & 33.3 & \textbf{33.5}          \\
TREC-NEWS       & \textbf{49.1} & 48.9 & 47.9 & 48.5          \\
Robust04         & 49.6 & 50.6 & 52.0 & \textbf{52.1}          \\
Touche-2020      & 31.8 & \textbf{36.2} & 34.2 & 33.4          \\
DBPedia          & 43.9 & \textbf{44.5} & 43.9 & 43.7          \\
SciFact          & 69.6 & 70.4 & \textbf{74.1} & \textbf{74.1}          \\ \midrule
\textbf{Avg (DL19, DL20)}  & 69.4 & 64.4 & 69.3 & \textbf{70.0} \\
\textbf{Avg (BEIR)}        & 48.8 & 49.4 & 49.7 & \textbf{49.9} \\ \bottomrule
%Avg(Full)       & 53.1 & 52.9 & 52.4 & {\ul 53.6} & \textbf{53.9} \\ \bottomrule
\end{tabular}

}
\caption{Comparison of \textsc{ListT5} against listwise (RankGPT) and pairwise (DuoT5) ranking models. The scores of RankGPT are from the paper, and the base model of RankGPT is GPT-3.5-turbo-0301. The best average is in bold. DuoT5 is applied on top 50 passages reranked by MonoT5. \textsc{ListT5} excels in both in-domain (DL19, DL20) and on the selected subset of BEIR.}
\label{table/rankgpt_duot5_deprecated}
\end{table}

\begin{comment}
\begin{table}[t]
    \resizebox{\columnwidth}{!}
    {
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{@{}l|ccccc@{}}
\toprule
\textbf{} &
  \multicolumn{1}{c}{MonoT5} &
  \multicolumn{1}{c}{DuoT5} &
  \multicolumn{1}{c}{RankGPT} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}l@{}}ListT5\\(Top1)\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}l@{}}ListT5\\(Top2)\end{tabular}} \\ \midrule
TREC-DL19       & 71.5 & 71.4 & 65.8 & 71.2 & 71.8          \\
TREC-DL20       & 67.0 & 67.4 & 62.9 & 67.3 & 68.1          \\ \midrule
TREC-COVID      & 78.3 & 80.1 & 76.7 & 76.7 & 78.3          \\
NFCorpus        & 35.7 & 35.0 & 35.6 & 35.5 & 35.6          \\
Signal-1M (RT)  & 32.0 & 31.4 & 32.1 & 33.3 & 33.5          \\
TREC-NEWS       & 48.0 & 49.1 & 48.9 & 47.9 & 48.5          \\
Robust04        & 53.4 & 49.6 & 50.6 & 52.0 & 52.1          \\
Touche-2020     & 29.6 & 31.8 & 36.2 & 34.2 & 33.4          \\
DBPedia         & 42.8 & 43.9 & 44.5 & 43.9 & 43.7          \\
SciFact         & 73.1 & 69.6 & 70.4 & 74.1 & 74.1          \\ \midrule
Avg(DL19, DL20) & 69.3 & {\ul 69.4} & 64.4 & 69.3 & \textbf{70.0} \\
Avg(BeIR)       & 49.1 & 48.8 & 49.4 & {\ul 49.7} & \textbf{49.9} \\ \bottomrule
%Avg(Full)       & 53.1 & 52.9 & 52.4 & {\ul 53.6} & \textbf{53.9} \\ \bottomrule
\end{tabular}

}
\caption{Comparison between listwise (RankGPT) and pairwise(DuoT5) ranking models with \textsc{ListT5}. The scores of RankGPT are from the paper, and base model of RankGPT is GPT-3.5-turbo-0301. The best average is in bold, and the second best is in underline. \textsc{ListT5} excels in both in-domain(DL19, DL20) and on the selected subset of BeIR, then any other baseline models.}
\label{table/rankgpt_duot5}
\end{table}
\end{comment}
